Deficit of primitive compositions in binary asteroids and pairs

Context. Small binary asteroid systems and pairs are thought to form through fission induced by spin up via the Yarkovsky-O'Keefe-Radzievskii-Paddack (YORP) effect. This process is expected to depend on their structural strength, hence composition. Aims. We aim to determine how taxonomic classes, used as a proxy for composition, distribute amongst binary asteroids and asteroid pairs compared to the general population. Methods. We compare the distribution of taxonomic classes of binary systems and pairs with that of a reference sample of asteroids. We build this sample by selecting asteroids to reproduce the orbital and size distribution of the binaries and pairs to minimize potential biases between samples. Results. A strong deficit of primitive compositions (C, B, P, D types) among binary asteroids and asteroid pairs is identified, as well as a strong excess of asteroids with mafic-silicate rich surface compositions (S, Q, V, A types). Conclusions. Amongst low mass, rapidly rotating asteroids, those with mafic-silicate rich compositions are more likely to form multiple asteroid systems than their primitive counterparts.

==> gfx/my_stats.tex <==
\newcommand{\nbTotBins}{402\xspace}    % All binaries
\newcommand{\nbTotPairs}{239\xspace}    % All Pairs
\newcommand{\nbBins}{279\xspace}    % used binaries
\newcommand{\nbPairs}{220\xspace}    % used pairs
\newcommand{\nbSpecPairs}{36\xspace}    % Pairs with spectra
\newcommand{\nbSpecBins}{127\xspace}    % Binaries with spectra
\newcommand{\nbDiamPairs}{65\xspace}    % Pairs with diameters from used 
\newcommand{\nbDiamBins}{220\xspace}    % Binaries with diameter from used
\newcommand{\nbPhotPairs}{85\xspace}    % Pairs with spectra
\newcommand{\nbPhotBins}{82\xspace}    % Binaries with spectra
\newcommand{\sizea}{0.28\xspace}    % a size
\newcommand{\sizee}{0.2\xspace}    % e size
\newcommand{\sizei}{10.0\xspace}    % i size
\newcommand{\sized}{1.5\xspace}    % d size
\newcommand{\Evlsig}{5.6\xspace}    % SQVA significance level
\newcommand{\Prmsig}{6.1\xspace}    % Primitive significance level

